Language Models Get a Gender Makeover: Mitigating Gender Bias with Few-Shot Data Interventions

Societal biases present in pre-trained large language models are a critical issue as these models have been shown to propagate biases in countless downstream applications, rendering them unfair towards specific groups of people. Since large-scale retraining of these models from scratch is both time and compute-expensive, a variety of approaches have been previously proposed that de-bias a pre-trained model. While the majority of current state-of-the-art debiasing methods focus on changes to the training regime, in this paper, we propose data intervention strategies as a powerful yet simple technique to reduce gender bias in pre-trained models. Specifically, we empirically show that by fine-tuning a pre-trained model on only 10 de-biased (intervened) training examples, the tendency to favor any gender is significantly reduced. Since our proposed method only needs a few training examples, our few-shot debiasing approach is highly feasible and practical. Through extensive experimentation, we show that our debiasing technique performs better than competitive state-of-the-art baselines with minimal loss in language modeling ability.

==> tables.tex <==
\usepackage{booktabs}
\usepackage{multirow}

\begin{document}
\begin{table}[]
\centering
\begin{tabular}{@{}clcccc@{}}
\toprule
\multirow{2}{*}{Type} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{StereoSet Scrores} & \multirow{2}{*}{Crow-S Scores} \\ \cmidrule(lr){3-5}
                           & \multicolumn{1}{c}{}      & SS              & LMS                                 & ICAT                                &                 \\ \midrule
\multirow{5}{*}{Baselines} & None                      & -               &                                     &                                     & -               \\ \cmidrule(l){2-6} 
                           & CDA-100                   & 60.022          & \multicolumn{1}{r}{83.466}          & \multicolumn{1}{r}{70.892}          & 56.107          \\ \cmidrule(l){2-6} 
                           & Dropout-100               & 60.529          & \multicolumn{1}{r}{83.811}          & \multicolumn{1}{r}{70.171}          & 55.977          \\ \cmidrule(l){2-6} 
                           & SentenceDebias-100        & 59.221          & \multicolumn{1}{r}{\textbf{84.166}} & \multicolumn{1}{r}{\textbf{71.308}} & 53.817          \\ \cmidrule(l){2-6} 
                           & INLP                      & \textbf{57.378} & \multicolumn{1}{r}{81.706}          & \multicolumn{1}{r}{69.119}          & \textbf{51.530} \\ \midrule
\multirow{4}{*}{Ours}      & Random-Phrase-Masking-10  & 58.002          & 76.893                              & \multicolumn{1}{r}{70.930}          & \textbf{52.797} \\ \cmidrule(l){2-6} 
                           & Random-Phrase-Masking-100 & \textbf{57.651} & 75.883                              & 68.025                              & 53.307          \\ \cmidrule(l){2-6} 
                           & Neutral-Masking-50        & 59.335          & 83.849                              & 73.918                              & 53.435          \\ \cmidrule(l){2-6} 
                           & Neutral-Masking-100       & 58.275          & \textbf{84.508}                     & \textbf{76.531}                     & 54.330          \\ \bottomrule
\end{tabular}
\end{table}
\end{document}

